Dont Add, dont Miss: Effective Content Preserving Generation from Pre-Selected Text Spans

The recently introduced Controlled Text Reduction (CTR) task isolates the text generation step within typical summarization-style tasks. It does so by challenging models to generate coherent text conforming to pre-selected content within the input text (``highlights''). This framing enables increased modularity in summarization-like tasks, allowing to couple a single CTR model with various content-selection setups and modules. However, there are currently no reliable CTR models, while the performance of the existing baseline for the task is mediocre, falling short of practical utility. Here, we address this gap by introducing a high-quality, open-source CTR model that tackles two prior key limitations: inadequate enforcement of the content-preservation constraint, and suboptimal silver training data. Addressing these, we amplify the content-preservation constraint in both training, via RL, and inference, via a controlled decoding strategy. Further, we substantially improve the silver training data quality via GPT-4 distillation. Overall, pairing the distilled dataset with the highlight-adherence strategies yields marked gains over the current baseline, of up to 30 ROUGE-L points, providing a reliable CTR model for downstream use.

==> tables/distilled_data_quality.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{0.4\columnwidth}{!}{%
\begin{tabular}{ll}
\hline
data type & R-L \\ \hline
original & 67.9 \\
GPT-4-generated & 79.0 \\ \hline
\end{tabular}%
}
\caption{Rouge-L results between manually and automatically annotated document-highlights-summary triplets. The automatic variants consist of such that were extracted using the original SuperPal model ("original") and those extracted with GPT-4. \avi{My rule of thumb is that table with only one single number column should always appear in-line text and not in a table. If you decide keeping this one, please bold the distilled result.}}
\label{tab:distilled_data_quality}
\end{table}

==> tables/gpt4_prompt_num_examples_tuning.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t!]
\centering
\resizebox{0.75\columnwidth}{!}{%
\begin{tabular}{ccccc}
\hline
\# examples & R-1 & R-2 & R-L & \multicolumn{1}{l}{METEOR} \\ \hline
1 & {\color[HTML]{333333} 81.0} & {\color[HTML]{333333} 66.0} & {\color[HTML]{333333} 73.0} & {\color[HTML]{333333} 76.3} \\
2 & {\color[HTML]{333333} \textbf{84.8}} & {\color[HTML]{333333} \textbf{68.4}} & {\color[HTML]{333333} \textbf{76.4}} & {\color[HTML]{333333} \textbf{81.4}} \\
3 & {\color[HTML]{333333} 80.2} & {\color[HTML]{333333} 64.1} & {\color[HTML]{333333} 71.8} & {\color[HTML]{333333} 76.6} \\
4 & {\color[HTML]{333333} 77.6} & {\color[HTML]{333333} 60.5} & {\color[HTML]{333333} 69.2} & {\color[HTML]{333333} 73.1} \\
5 & {\color[HTML]{333333} 81.6} & {\color[HTML]{333333} 64.5} & {\color[HTML]{333333} 71.0} & {\color[HTML]{333333} 77.2} \\ \hline
\end{tabular}%
}
\caption{ROUGE and METEOR results on 50 instances from the CTR development set of GPT-4 models, for different numbers of in-context examples in the prompt.}
\label{tab:gpt4_prompt_num_examples_tuning}
\end{table}
